Using Model Checking to Generate Test Cases for Android Applications

The behavior of mobile devices is highly non deterministic and barely predictable due to the interaction of the user with its applications. In consequence, analyzing the correctness of applications running on a smartphone involves dealing with the complexity of its environment. In this paper, we propose the use of model-based testing to describe the potential behaviors of users interacting with mobile applications. These behaviors are modeled by composing specially-designed state machines. These composed state machines can be exhaustively explored using a model checking tool to automatically generate all possible user interactions. Each generated trace model checker can be interpreted as a test case to drive a runtime analysis of actual applications. We have implemented a tool that follows the proposed methodology to analyze Android devices using the model checker Spin as the exhaustive generator of test cases.

==> eptcsdata.tex <==
\providecommand{\firstpage}{7}
\providecommand{\publicationstatus}{A.K. Petrenko, B.-H. Schlingloff, N. Pakulin (Eds.):\\
Tenth Workshop on Model-Based Testing (MBT 2015)\\
EPTCS 180, 2015, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.180.1}{10.4204/EPTCS.180.1}}
\pdfoutput=1

